Tracking Adiabaticity in Non-Equilibrium Many-Body Systems: The Hard Case of the X-ray Photoemission in Metals

The level of adiabaticity determines many properties of time-dependent quantum systems. However, a reliable and easy-to-apply criterion to check and track it remains an open question, especially for complex many-body systems. Here we test techniques based on metrics which have been recently proposed to quantitatively characterize and track adiabaticity. We investigate the time evolution of x-ray photoemission in metals, which displays a strongly out-of-equilibrium character, continuum energy spectrum, and experiences the Anderson orthogonality catastrophe: a nightmarish scenario for this type of test. Our results show that the metrics-based methods remains valid. In particular, we demonstrate that the natural local density distance is able not only to track adiabaticity, but also to provide information not captured by the corresponding Bures' or trace distances about the system's dynamics. In the process, we establish an explicit upper limit for this local density distance in terms of the trace distance, and derive a simple analytical solution that accurately describes the time evolution of a Fermi gas with a localized scattering potential for a large range of parameters. We also demonstrate that, for x-ray photoemission, the quantum adiabatic criterion, as commonly used, fails to predict and track adiabaticity. The local particle density is typically much simpler to compute than the corresponding quantum state and it is experimentally measurable: this makes the method tested extremely appealing.

==> Old_Versions/Pieces_of_Text.tex <==
The wave function metrics defined by Eq.\eqref{BR} and \eqref{TR} can flag this behavior. Indeed, for example, Eq. \eqref{AOC} would give a Bures distance of
$D_{\rho}^{B} \sim \sqrt{2}\sqrt{1- \left(\frac{2\tau}{\Delta\varepsilon}\right)^{-\left({\frac{\delta}{\pi}}\right)^2}}$ immediately after the localized scattering potential appears.

However, what happens with the local density distance in this case? The occupation of each site is a local property and takes time to change. In fact, we can compute the occupation of the $l$-th eNRG site as a function of time as
\begin{eqnarray}\label{ldsq}
n_l(t) =\sum_{\substack{p,h,k \\ \varepsilon_k < \varepsilon_F}}\langle g_p| f_l\rangle\langle f_l|g_h\rangle\langle \tilde{g}_k | g_p \rangle\langle g_h | \tilde{g}_k \rangle e^{-i(\varepsilon_p-\varepsilon_h)t/\hbar}. \hspace{0.25 cm}
\end{eqnarray}
Where $\ket{g_p}$ and $\ket{g_h}$ represents single-particle eigenstates for the final Hamiltonian with energies $\varepsilon_p$ and $\varepsilon_h$, and $\ket{\tilde{g}_k}$ the single-particle eigenstates for the initial Hamiltonian.

The works in \cite{PhysRev.178.1097, Doniach_1970} have demonstrated that x-ray photoemission exhibits an experimentally observed power law in energy spectra, known as the Doniach-Sunjic law. This law is a function of the phase shift of the scattering potential, which for the tight-binding model is given by $\delta(t) = \rm{atan}\left(-\rho K(t) \right)$, with $\rho = \frac{1}{2\tau}$. Since $K(t)$ represents a localized scattering potential in a fermionic system, the OAC is observed and plays a important role in the physics of this phenomenon \cite{PhysRev.178.1097, Doniach_1970, PhysRevB.24.4863}.


If the scattering potential changes continuously in time, the modulus of the projection between the ground state in the instant $t$ and $t+dt$ is one since the phase shift between then tends to zero. In this scenario, only one-particle-hole excitation of each instantaneous eigenstate is significant. Therefore, when the scattering potential changes rapidly, the one-particle-hole excited states redistribute the occupation from the instantaneous ground state to two-particle-hole excitations, and so on. This diffusion-like process results in a rapid reduction of ground state occupancy, leading the system to deviate from adiabaticity. But if the scattering potential changes slowly, only low-energy one-particle-hole excitations can be occupied. And if this change is slowly enough, the system remains in the instantaneous ground state and the system dynamic is adiabatic. 

The real-space Numerical Renormalization Group (eNRG) method starts from a 1D tight-binding chain with hopping parameter $\tau$. The eNRG procedure considers cells comprising  $\lambda^n$ sites (n=0,1,2,3...), where $\lambda>1$, all those sites are lumped together in a definite single operator $f_n$, and the resulting hooping becomes $\tau_n=\tau\lambda^{-n-1/2}$. Also introduced is a second discretization parameter $\zeta$ (offset), specifically the firsts $\zeta$ sites that are treated individually \cite{Ferrari2022}.

The computed photocurrent combines physical and artificial oscillations as a function of time. Unphysical oscillations are defects of the eNRG discretization. In order to eliminate such oscillations, we rely on a smoothing procedure, where we let $\tau_n\rightarrow \tau_n \lambda^{\theta}$, as prescribed by the $w-$trick \cite{Ferrari2022}. Sequences of $N_e$ $\theta$ can be defined by two alternative prescriptions: \textbf{(1)} uniform distribution range from $\theta\in[-1/2,1/2]$; \textbf{(2)} random distribution as in reference \cite{Micklitz2022}. The resulting photocurrents are average over $\theta$. In addition, we average the photocurrent over two successive $\zeta$, typically $\zeta=3$ and $4$.

We can observe that the analytical solution yields results close to the eNRG even when the evolution is far from adiabaticity. Close to adiabaticity, the results from both methods align.




\subsection{Comparing the distances}

Here we initially fixed the Wilson chain size as $N=9$ and set $\lambda = 2$. We also set $ dt = 0.01$ to ensure that $ (\frac{K_T}{T} \Delta t)^2  \ll 1 $. All The time-like parameters/variables are in units of $({\hbar}/{\tau})$. Subsequently, we computed the metrics for various combinations of the maximum scattering potential $K_T$ and the time scale $T$. The $T=0$ case correspond to the usual sudden quench analysis.

Subsequently, we computed the metrics for various combinations of the maximum scattering potential $K_T$ and the time scale $T$. The $T=0$ case correspond to the usual sudden quench analysis.

First, we aim to show that the trace distance can be a superior limit of the density distance \eqref{NR}. The primary results of this analysis can be found in Figures \ref{fig:Results1} for weak amplitudes and Figure \ref{fig:Results2} for strong amplitudes. We observe that in all cases the density distance $D_n(t) < D_\rho^T(t)$, which is in line with our expectations, as we have established $D_n \le 2 D_\rho^T$. However, it is worth mentioning that the gap between the numerical and this upper limit is larger than we initially anticipated. Nevertheless, this observation remains interesting, as it offers a simple way to determine an upper limit.

After these initial discussions about the analytical calculations, we will divide the Numerical Results section into three parts. This division will allow us to discuss different topics and use different parameters without confusion. In the first part, we will compare the wave function distances and density distances for various $K_T$ and $T$. In the second part, we will discuss how the metrics can track adiabaticity. In the last part, we discuss whether the metrics can capture the OAC and how it is related to adiabaticity.

\begin{figure}[htb!]
    \centering
    \includegraphics[scale=0.255]{figures/dis025.pdf}
    \caption{Time evolution of the metrics for weak maximum scattering amplitudes $K$ computed with $K_T = -0.1$ (Right) and $K_T = -0.2$ (Left) for different time scales $T$.}
    \label{fig:Results1}\label{fig:Results2}
\end{figure}

Let us start with the wave function metrics, the time evolution of these distances follow the value of the instantaneous ground state transition probability $|\bra{\varphi_0(t)}\ket{\Psi(t)}|^2$ as we discuss before.
The time evolution of the Bures $D_\rho^B (t)$ and the trace distance $D_\rho^T (t)$ are in the results \ref{fig:Results1} and \ref{fig:Results2} for different time scales $T$ and scattering amplitudes $K_T$. It starts at $t=0$ with the system in the initial ground state. For $0<t<T$ the Hamiltonian changes linearly, the initial ground state is no longer an eigenstate, and the excited states start to be occupied. If the evolution is slow enough, the system predominantly stays in the instantaneous ground state then the distances is small. However, with faster changes, the excited states increasingly contribute, causing the increase of the distances. For $t > T$ the Hamiltonian stop to change and the transition probability for each eigenstate of $\hat H(T)$ remains the same, so after this point, the metrics become a horizontal line.

The local density distance does not have a directly visualization as the above metrics; however, we find a superior limit related with the trace distance and also exist a connection with the Bures distance. If $\hat{H}(t)$ change slowly enough the system have time for the particles distribution follow the adiabatic distribution and the distance is small. But if the Hamiltonian changes fast, the system can not follow the adiabatic distribution, then the distance is bigger. So seems like this metric has the same information as the wave function metrics we discuss above.

Using the results in Figures \ref{fig:Results1} and \ref{fig:Results2} we can see that analyzing the maximum amplitude for the metrics that the three distances, Bures, trace, and density, contain the same information. In cases involving faster and/or stronger scattering potentials, we can observe an increase in all these metrics. This suggests that the excited states of the system are being occupied. In contrast, for slowly growing potentials or weak amplitudes, the metrics remain small, indicating that the wave function is closer to the instantaneous ground state. Also, for small times, all the metrics behave similar. This thought can be reinforced by the results in Figure when we plot the relationship between Bures distance and density distance. In the results for slowly growing potentials or weak amplitudes, the density distance and the Bures distance exhibit almost linear behavior between them. Nevertheless, for scenarios involving strong scattering potentials and/or rapid time scales, the density distance does not behave linearly with the Bures distance anymore. By observing situations where the Bures distance versus density distance curve exhibits a linear behavior $D_n \approx m D_\rho^B$ (in this case $m \approx 0.45$) it becomes possible to determine the adiabatic density distance criteria using the Bures distance criteria $D_n < 0.045$.

%\begin{center}
%\begin{figure}[hbt!]
%    \centering
%    \includegraphics[scale=0.255]{figures/metrica_metrica.pdf}
%    \caption{The relationship between the Bures distance and the density distance computed for different values of the scattering potential $K_T$ and for different time scale $T$.}
%    \label{fig:Results3}
%\end{figure}   
%\end{center}

However, it becomes evident that for longer times, if the scattering potential grows rapidly or is strong, the differences in behavior between the density distance and the Bures distance become more expressive. In some combinations of $K_T$ and $T$, for example $K_T=-5$ and $T$ $\{10,50,100\}$, as shown in Fig. \ref{fig:Results2}, the density distance reaches a maximum value before the time scale $T$. In contradiction, the wave function metrics always get the maximum value at the exact point that $-K_T$ is maximum. Since for $t>T$ the Hamiltonian does not change, the wave function metrics become constant after this point, but the density distance is still changing in time.

The adiabaticity criteria we are employing here is that the ground state transition probability $|c_0|^2$ should remain above $0.99$. This criterion aligns with the maximum values of Bures and the trace distances defined by Skelt, which are, respectively, $D_\rho^B < 0.1$ and $D_\rho^T < 0.1$.

Finally, we discuss how to classify adiabaticity in this MB system using the previously discussed metrics. Once again, it is essential to emphasize that our adiabaticity criterion remains on maintaining the ground state transition probability $|c_0|^2$ above the threshold of $0.99$ which corresponds to the Bures and trace distance bellow $0.1$ and as we find, the density distance bellow $0.045$. We can see in the results for $K_T = -0.1$ found in Figure \ref{fig:Results1} that both the Bures and Trace distances remains bellow $0.1$ even for $T=0$, the sudden creation of the scattering potential. Then, for $K_T = -0.1$ and of course any $ 0 > K_T > -0.1$ the time evolution is adiabatic for any $T$. However, this situation changes for $K_T = -0.2$ as shown in Figure \ref{fig:Results2}. In this particular scenario, for time scales $T \le 50$, the system behaves as non-adiabatic, as indicated by $D_\rho^T > 0.1$. However, for $T \approx 100$, $D_\rho^T < 0.1$, signifying that the dynamics is adiabatic. We can observe that the same analyses can be performed with the density metrics to obtain the same conclusions. These findings imply the presence of a critical time scale. Below this time scale threshold, the dynamics is rapid, leading to a non-adiabatic system behavior. Although above this critical value, the time evolution slows down, resulting in an adiabatic system behavior. In Figure \ref{fig:Results2} (Right), we displayed the results for $K_T = -1$. Given the exceptionally strong scattering potential, the computed time scales are significantly smaller than $T_C (K_T =-1)$, resulting in non-adiabatic behavior for all values of $T$ we computed.

The discussion about adiabaticity we did in the last subsection is very useful to track the behavior of the time evolution of a quantum many-body system, and they work exceptionally well for a finite size system. However, when we deal with macroscopic systems they have the order of $10^{23}$ atoms and since the X-ray photoemission phenomena creates a localized scattering potential, the Anderson's Orthogonality Catastrophe appear. So here is very important discuss about the size of the chain, since it could drastically interfere in ones results more then just, even more then non physical oscillations which naturally happens in discretized results. As we show in the Eq. the effective number of sites in your chain is related to the discretization parameter $\Lambda$. We can increase our effective chain by increasing the value of this parameter. Since our Fermi Level is fixed in zero, then the number of electrons in our system is the half of the number of sites. So, in this subsection we want to change the effective chain size to see the impact of this change on the metrics.

Also, for $T<160$ the QAC underestimate the condition for adiabaticity and for $T>160$ it considers points with nonadiabatic dynamics as adiabatic.



To investigate scenarios involving small gaps / long measurement time scales, the metallic band can be discretized logarithmically \cite{PhysRevB.24.4863,PhysRevB.49.11986, PhysRevB.106.075129, RevModPhys.47.773, RevModPhys.80.395}. Then, by computing the time evolution of the x-ray photoemission problem, it is possible to track adiabaticity using metrics for both the gapped energy spectrum and the 



(I) About the metrics; It can be used for track Adiabaticity;

(II) About the analytical result; Have results good enough in the interested regime;

(III) About tracking adiabaticity; This procedure allow us to study adiabaticity in the continuum spectra limit.

(IV) About the density distance; Have similar information for short times and different for longer times; It can be also used to track adiabaticity for this system.
